Security of Language Models for Code: A Systematic Literature Review

Language models for code (CodeLMs) have emerged as powerful tools for code-related tasks, outperforming traditional methods and standard machine learning approaches. However, these models are susceptible to security vulnerabilities, drawing increasing research attention from domains such as software engineering, artificial intelligence, and cybersecurity. Despite the growing body of research focused on the security of CodeLMs, a comprehensive survey in this area remains absent. To address this gap, we systematically review 67 relevant papers, organizing them based on attack and defense strategies. Furthermore, we provide an overview of commonly used language models, datasets, and evaluation metrics, and highlight open-source tools and promising directions for future research in securing CodeLMs.

==> tables/adversarial_attacks_black_box.tex <==
\begin{table*}[!t]
    \centering
    \scriptsize
    \caption{A summary of existing black-box adversarial attacks on \abbr{}s.}
    \label{tab:adversarial_attacks_black_box}
    \scalebox{0.82}{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        
        Attack Technique & Year & Venue & Attack Type & Target Models & Target Tasks \\

        \midrule 

        Quiring et al.~\cite{2019-Misleading-Authorship-Attribution} & 2019 & USENIX Security & Black-box attack & Random Forest, LSTM & Authorship attribution \\

        \midrule 

        Matyukhina et al.~\cite{2019-Adversarial-Authorship-Attribution-in-Open-Source-Projects} & 2019 & CODASPY & Black-box attack & N-grams & Authorship attribution\\

        \midrule

        SCAD~\cite{2021-A-Practical-Black-Box-Attack-on-Source-Code-Authorship-Identification-Classifiers} & 2021 & TIFS & Black-box attack & \makecell[c]{Random Forest, RNN} & Authorship attribution\\

        \midrule

        STRATA~\cite{2020-STRATA} & 2020 & ArXiv & Black-box attack & Code2Seq & Method name prediction \\

        \midrule 

        MHM~\cite{2020-MHM} & 2020 & AAAI & Black-box attack & \makecell[c]{BiLSTM, ASTNN} & Function classification\\

        \midrule 

        Pour et al.~\cite{2021-A-Search-Based-Testing-Framework} & 2021 & ICST & Black-box attack & \makecell[c]{Code2Vec, Code2Seq\\CodeBERT} & \makecell[c]{Method name prediction\\Code description\\Code search, Code summarization} \\

        \midrule 

        QMDP~\cite{2021-Generating-adversarial-examples-of-source-code-classification-models-via-q-learning-based-markov-decision-process} & 2021 & QRS & Black-box attack & \makecell[c]{LSTM, ASTNN} & Function classification\\

        \midrule 

        Ferretti et al.~\cite{2021-Deceiving-neural-source-code-classifiers-finding-adversarial-examples-with-grammatical-evolution} & 2021 & GECCO & Black-box attack & Random Forest, CNN & Vulnerability detection\\

        \midrule 

        Anand et al.~\cite{2021-Adversarial-Robustness-of-Program-Synthesis-Models} & 2021 & CoRR & Black-box attack & \makecell[c]{SketchAdapt\\SAPS, Seq2Tree} & Code generation\\

        \midrule 

        ACCENT~\cite{2022-Adversarial-Robustness-of-Deep-Code-Comment-Generation} & 2022 & TOSEM & Black-box attack & \makecell[c]{LSTM, GNN\\CSCG, Rencos} & Code summarization \\

        \midrule 

        ALERT~\cite{2022-Natural-Attack-for-Pre-trained-Models-of-Code} & 2022 & ICSE & Black-box attack & \makecell[c]{CodeBERT\\GraphCodeBERT} & \makecell[c]{Vulnerability detection\\Clone detection\\Authorship attribution} \\

        \midrule 

        Li et al.~\cite{2022-RoPGen} & 2022 & ICSE & Black-box attack & DL-CAIS, PbNN & Authorship attribution \\

        \midrule 

        TABS~\cite{2022-TABS} & 2022 & EMNLP & Black-box attack & CodeBERT & \makecell[c]{Code classification\\Code search}\\

        \midrule 

        FuncFooler~\cite{2022-funcfooler} & 2022 & ArXiv & Black-box attack & \makecell[c]{RNN\\PV-DM\\Transformer} & Binary similarity detection \\

        \midrule 

        Mercuri et al.~\cite{2023-Evolutionary-Approaches-for-Adversarial-Attacks-on-Neural-Source-Code-Classifiers}& 2023 & Algorithms  & Black-box attack & CNN & \makecell[c]{Vulnerability detection}\\

        \midrule 
        
        CodeAttack~\cite{2023-CodeAttack} & 2023 & AAAI & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT\\} & \makecell[c]{Code transformation\\Code repair\\Code summarization} \\

        \midrule 

        DaK~\cite{2023-Discrete-Adversarial-Attack} & 2023 & PLDI & Black-box attack & \makecell[c]{Code2Vec, GGNN\\CodeBERT} & Variable misuse prediction \\

        \midrule 

        GraphCodeAttack~\cite{2023-Adversarial-Attacks-on-Code-Models} & 2023 & ArXiv & Black-box attack & \makecell[c]{CodeBERT\\GraphCodeBERT} &  \makecell[c]{Authorship attribution\\Vulnerability detection\\Clone detection} \\

        \midrule 

        ADVULCODE~\cite{2023-AdVulCode} & 2023 & Electronics & Black-box attack & \makecell[c]{BiGRU, GGNN\\BiLSTM} & Vulnerability detection \\

        \midrule 

        DIP~\cite{2023-DIP} & 2023 & ACL & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT} & \makecell[c]{Clone detection\\Vulnerability detection\\Authorship attribution} \\

        \midrule 

        RNNS~\cite{2023-RNNS} & 2023 & ArXiv & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT} & \makecell[c]{Clone detection\\Vulnerability detection\\Authorship attribution\\Function classification} \\

        \midrule 

        SHIELD~\cite{2023-SHIELD} & 2023 & CoRR & Black-box attack & \makecell[c]{CNN, CSFS, DL-CAIS} & Authorship attribution\\

        \midrule 

        CODA~\cite{2023-Code-Difference-Guided-Adversarial-Example-Generation-for-Deep-Code-Models} & 2023 & ASE & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT} & \makecell[c]{Vulnerability detection\\Authorship attribution\\Function classification\\Clone detection, Defect detection}\\

        \midrule

        CodeBERT-Attack~\cite{2023-CodeBERT-Attack} & 2023 & JSEP & Black-box attack & \makecell[c]{LSTM, CodeBERT\\GraphCodeBERT} & \makecell[c]{Function classification\\Clone detection}\\

        \midrule 

        RADAR~\cite{2024-radar} & 2024 & TOSEM & Black-box attack & \makecell[c]{CodeGPT\\PLBART, CodeT5} & \makecell[c]{Code generation} \\
        
        \midrule

        AWAL et al.~\cite{2024-investigating-adv} & 2024 & CoRR & Black-box attack & \makecell[c]{Logistic Regression\\Multi-Layered Perceptron\\Gradient Boosting Classifier\\Decision Tree, AdaBoost\\Random Forest, Bagging} & \makecell[c]{Defect detection\\Clone detection\\Code classification}\\

        \midrule 

        DeceptPrompt~\cite{2023-Deceptprompt} & 2023 & CoRR & Black-box attack & \makecell[c]{CodeLlama, StarChat\\WizardCoder} & \makecell[c]{Code generation\\Vulnerability detection}\\

        \midrule 

        STRUCK~\cite{2024-STRUCK} & 2024 & CollaborateCom & Black-box attack & \makecell[c]{LSTM, GRU, GCN\\GGNN, CodeBERT\\GraphCodeBERT\\UniXcoder} & \makecell[c]{Function classification\\Defect detection}\\

        \midrule 

        CodeTAE~\cite{2024-CodeTAE} & 2024 & TIFS & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT} & \makecell[c]{Authorship attribution\\Clone detection\\Defect detection}\\

        \midrule 

        MoAA~\cite{2024-MOAA} & 2024 & FSE & Black-box attack & \makecell[c]{CodeBERT, CodeT5\\GraphCodeBERT} & \makecell[c]{Defect detection, Clone detection\\Authorship attribution\\Code translation\\Code summarization}\\

        \midrule 

        MalwareTotal~\cite{2024-MalwareTotal} & 2024 & ICSE & Black-box attack & \makecell[c]{EMBER, MalConv\\AMS A/B, ClamAV} & Malware detection\\

        \midrule

        CARL~\cite{2024-carl} & 2024 & TOSEM & Black-box attack & \makecell[c]{CodeBERT\\CodeT5\\UniXcoder\\GraphCodeBERT\\CodeGeeX2} & \makecell[c]{Code summarization\\Code translation\\Code refinement} \\
        
        \bottomrule
    \end{tabular}
    }
    }
\end{table*}

